An Instability in the Radiative Ionization of Atomic Hydrogen/Helium Gas

We show that the process of photoionizing a gas of atomic hydrogen and helium by line radiation whose energy is slightly above the helium single-ionization threshold is unstable if the helium fraction by number is less than approximately one half. However, in the two scenarios we consider here, based on the Decaying Dark Matter (DDM) model of cosmological reionization, there is no significant growth. In the first scenario we consider ionization and recombination to be approximately in equilibrium. This is relevant to high photon flux rates and early reionization, but in that case the heating is balanced by Compton cooling, which is very stabilizing. In the second scenario we ignore recombination. This is relevant to low photon flux rates or to the last stage of the reionization. In that case there is too little growth on a cosmological time scale to be significant.

==> he2-table-text.tex <==
%auto-ignore
\begin{deluxetable}{|ll|}
  \tablewidth{0pt}
  \tablecaption{Symbols}
  \tablehead{\colhead{Symbol/Value}&\colhead{Explanation}}
  \startdata

  \parbox[t]{1.6 in}{
    $h$
    }&
  \parbox[t]{3.6 in}{
    The Hubble Parameter in units of 100 km/s/Mpc.
    }\nl

  \parbox[t]{1.6 in}{
    $\omega_g =-i \omega$
    }&
  \parbox[t]{3.6 in}{
    Instability growth rate.
    }\nl

  \parbox[t]{1.6 in}{
    $\vec{k}$
    }&
  \parbox[t]{3.6 in}{
    Wave vector in Fourier decomposition.
    }\nl

  \parbox[t]{1.6 in}{
    $k\equiv|k|$
    }&
  \parbox[t]{3.6 in}{
    Wave number (inverse of size scale).
    }\nl

  \parbox[t]{1.6 in}{
    $n$
    }&
  \parbox[t]{3.6 in}{
    Total spatial density of hydrogen plus helium nuclei
    (neutral and ionized).
    }\nl

  \parbox[t]{1.6 in}{
    $u={1 \over \gamma -1}(1+\chi)n T_m$
    }&
  \parbox[t]{3.6 in}{
    Internal thermal energy of the gas.
    }\nl

  \parbox[t]{1.6 in}{
    $\gamma = 5/3$
    }&
  \parbox[t]{3.6 in}{
    Adiabatic expansion coefficient.
    }\nl

  \parbox[t]{1.6 in}{
    ${\cal P}$
    }&
  \parbox[t]{3.6 in}{
    Heat input per unit volume.
    }\nl

  \parbox[t]{1.6 in}{
    $v_s$
    }&
  \parbox[t]{3.6 in}{
    The unperturbed speed of sound.
    }\nl

  \parbox[t]{1.6 in}{
    $\mu={Y_p \over 4 - 3 Y_p} \approx 0.073$
    }&
  \parbox[t]{3.6 in}{
    Fraction by number of helium atoms ($Y_p \approx .24$ is used here).
    }\nl

  \parbox[t]{1.6 in}{
    $\omega_u = {\cal P}_u\\
     \omega_k = v_s k\\
     \omega_n = -{{\cal P}_n n \over\gamma u}$
    }&
  \parbox[t]{3.6 in}{
    Miscelaeous rates.
    }\nl

  \parbox[t]{1.6 in}{
    $p_1=0.554$
    }&
  \parbox[t]{3.6 in}{
    Number of photons produced in a two-photon decay of the He $2 {}\,^1\!S$ state
    which can ionize H.
    }\nl

  \parbox[t]{1.6 in}{
    $n_{\gamma 0}, n_{\gamma 1}$, etc.}&
  \parbox[t]{3.6 in}{
    Spatial density 
    of photons with energy $E_0, E_1, $ etc.
    }\nl

  \parbox[t]{1.6 in}{
    $n_{\rm He\,II}=n\mu \chi_{\rm He}$
    }&
  \parbox[t]{3.6 in}{
    Number density of ionized helium.
    }\nl

  \parbox[t]{1.6 in}{
    $n_{\rm He\,I}=n\mu(1- \chi_{\rm He})$
    }&
  \parbox[t]{3.6 in}{
    Number density of neutral helium.
    }\nl

  \parbox[t]{1.6 in}{
    $n_{\rm H\,II}=n(1-\mu) \chi_{\rm H}$
    }&
  \parbox[t]{3.6 in}{
    Number density of ionized hydrogen.
    }\nl

  \parbox[t]{1.6 in}{
    $n_{\rm H\,I}=n(1-\mu)(1- \chi_{\rm H})$
    }&
  \parbox[t]{3.6 in}{
    Number density of neutral hydrogen.
    }\nl

  \parbox[t]{1.6 in}{
    $n_e=n_{\rm He\,II}+n_{\rm H\,II}=n \chi$
    }&
  \parbox[t]{3.6 in}{
    Number density of electrons.
    }\nl

  \parbox[t]{1.6 in}{
    $\chi_{\rm He}$
    }&
  \parbox[t]{3.6 in}{
    Fractional ionization of helium.
    }\nl

  \parbox[t]{1.6 in}{
    $\chi_{\rm H}$
    }&
  \parbox[t]{3.6 in}{
    Fractional ionization of hydrogen.
    }\nl

  \parbox[t]{1.6 in}{
    $\chi = \mu  \chi_{\rm He}+(1-\mu) \chi_{\rm H}$
    }&
  \parbox[t]{3.6 in}{
    Fractional ionization of all species combined.\\
    }\nl

  \parbox[t]{1.6 in}{
  $\sigma_{\rm H}(E)=6.30\times{10}^{-18}\times\\
  \;\;x^{-4} {e^{4(1-y \, {\rm arccot}(y))} \over 1-e^{-2\pi y}}{\rm cm}^2\\
  \mbox{\hspace{10pt}}x={E \over {\rm Ry}}\\
  \mbox{\hspace{10pt}}y={1 \over \sqrt{x-1}}$
  }&
  \parbox[t]{3.6 in}{
    Absorption cross section of hydrogen for
    photons with energy $E$.\tablenotemark{b}
    }\nl

\ifnum\outtype=1
\tablebreak
\fi

  \parbox[t]{1.6 in}{
  $\sigma_{\rm H \, \mit m}=\sigma_{\rm H}(E_m)$
  }&
  \parbox[t]{3.6 in}{
    Absorption cross section of hydrogen for
    photons with energy $E_m$, for some $m$.
    }\nl

  \parbox[t]{1.6 in}{
    $\sigma_{\rm He \, \mit m}=\sigma_{\rm H \, \mit m} \times \\
    \;\;(6.53{E_m \over E_1}-0.22)$
  }&
  \parbox[t]{3.6 in}{
   Absorption cross section of helium for
   photons with energy $E_m$, for some $m$.\tablenotemark{c}
   }\nl

  \parbox[t]{1.6 in}{
    $\alpha_{{\rm H} 2}=2.59\times{10}^{-13}{{cm}^3 \over s}$
    }&
  \parbox[t]{3.6 in}{
    Recombination coeff.\ for H to
    all excited levels.\tablenotemark{a}
    }\nl

  \parbox[t]{1.6 in}{
    ${\alpha}_{{\rm He} 2}=2.73\times{10}^{-13}{{cm}^3 \over s}$
    }&
  \parbox[t]{3.6 in}{
    Recombination coeff.\ for He to
    all excited levels.\tablenotemark{a}
    }\nl

  \parbox[t]{1.6 in}{
    ${\alpha}_{{\rm He} 2 {}\,^1\!P} = {2 \over 3}
    \left({1 \over 4}\alpha_{{\rm He} 2}\right)$
    }&
  \parbox[t]{3.6 in}{
    Recombination coeff.\ for He to
    excited singlet levels which cascade to the $2{}^1\!P$ state.
    }\nl

  \parbox[t]{1.6 in}{
    ${\alpha}_{{\rm He} 2 {}\,^1\!S} = {1 \over 3}
    \left({1 \over 4}\alpha_{{\rm He} 2}\right)$
    }&
  \parbox[t]{3.6 in}{
    Recombination coeff.\ for He to
    excited singlet levels which cascade to the $2 {}\,^1\!S$ state.
    }\nl

  \parbox[t]{1.6 in}{
    ${\alpha}_{{\rm He} 2 {}\,^3\!P} = {3 \over 4}\alpha_{{\rm He} 2}$
    }&
  \parbox[t]{3.6 in}{
    Recombination coeff.\ for He to all
    excited triplet levels (all of which lead to the $2 {}\,^3\!P$ state).
    }\nl

  \parbox[t]{1.6 in}{
    ${\alpha}_{\rm He 1}=1.59\times{10}^{-13}{{cm}^3 \over s}$
    }&
  \parbox[t]{3.6 in}{
    Recombination coeff.\ for He to
    ground.\tablenotemark{a}
    }\nl

  \parbox[t]{1.6 in}{
    $\Re = n_\nu / \tau_\nu$
    }&
  \parbox[t]{3.6 in}{
    Rate of production of primary photons.
    }\nl

  \parbox[t]{1.6 in}{
    $\delta = {E_0 \over E_1} - 1$
    }&
  \parbox[t]{3.6 in}{
    Dimensionless excess energy of ionization photon.
    }\nl

  \parbox[t]{1.6 in}{
    $\phi={T_m \over T_\gamma}$
    }&
  \parbox[t]{3.6 in}{
    Ratio of the matter temperature to the radiation temperature.
    }\nl

  \parbox[t]{1.6 in}{
    $z'=1+z$}&
  \parbox[t]{3.6 in}{
    Inverse of the cosmic scale factor.
    }\\

  \parbox[t]{1.6 in}{
    $\tau_{24} = \tau_\nu / 10^{24} {\rm sec}$
    }&
  \parbox[t]{3.6 in}{
    Neutrino decay rate in units of $10^{24}$ seconds.
    }\nl
\enddata

\tablenotetext{a}{From Osterbrock 1989 % ApJ says no paren in table citations.
 \nocite{Osterbrock:1} for $T=10000K$.}
\tablenotetext{b}{From Spitzer 1978\nocite{Spitzer}.}
\tablenotetext{c}{From Brown 1971\nocite{Brown:photoionization}.}
\end{deluxetable}

\begin{deluxetable}{|lll|}
  \tablewidth{0pt}
  \tablecaption{Energy Values}
  \tablehead{\colhead{Sym.}&\colhead{Value}&\colhead{Explanation}}
  \startdata
  $E_0$&\nodata&Primary photon energy\\
  $E_1$&24.6 eV\tablenotemark{a}&Ionization energy of He\\
  $E_2$&19.8 eV\tablenotemark{a}&Energy of He $2 {}\,^3\!P$\\
  $E_3$&21.2 eV\tablenotemark{a}&Energy of He $2 {}\,^1\!P$\\
  $E_4$&20.6 eV\tablenotemark{a}&Energy of He $2 {}\,^1\!S$\\
  $E_5$&16.1 eV\tablenotemark{b}&Avg. energy of $\gamma$ absorbed by H in 2$\gamma$
  decay of He $2 {}\,^1\!S$\\
  ${\rm Ry}$&13.6 eV&H ionization energy\\
  $\Delta E$&$E_0-{\rm Ry}$&Energy deposited in a direct H ionization\\
  $\Delta E_{\rm He}$&$E_0-E_1$&Energy deposited in a He ionization\\
  \enddata
  \label{ETable}
  \tablenotetext{a}{From Osterbrock 1989. % ApJ says no paren in table citations.
    \nocite{Osterbrock:1}}
  \tablenotetext{b}{See Appendix~C.}
\end{deluxetable}
% Local Variables:
% TeX-master: "he2"
% End:

